Numerical simulations of the kappa-mechanism with convection

A strong coupling between convection and pulsations is known to play a major role in the disappearance of unstable modes close to the red edge of the classical Cepheid instability strip. As mean-field models of time-dependent convection rely on weakly-constrained parameters, we tackle this problem by the means of 2-D Direct Numerical Simulations (DNS) of kappa-mechanism with convection. Using a linear stability analysis, we first determine the physical conditions favourable to the kappa-mechanism to occur inside a purely-radiative layer. Both the instability strips and the nonlinear saturation of unstable modes are then confirmed by the corresponding DNS. We next present the new simulations with convection, where a convective zone and the driving region overlap. The coupling between the convective motions and acoustic modes is then addressed by using projections onto an acoustic subspace.

==> Makefile <==
# $Id: Makefile,v 1.2 2009/09/08 07:42:33 tgastine Exp $
# Makefile for generating different output formats of the $(FILE) inspired
# from the Pencil Code one used to build the manual.
#
# Usage:
#  make
#  make $(FILE).pdf
#  make clean
#
# ------------------
FILE             = proceeding
LATEX            = latex -src
DVIPS            = dvips
BIBTEX           = bibtex
PS2PDF           = ps2pdf14 -sPAPERSIZE=a4 -dPDFSETTINGS=/prepress
MAY_HAVE_CHANGED = 'may have changed. Rerun to get'
MAY_NO_BIBTEX    = 'undefined citations'
# ------------------
.SUFFIXES:            # clear all generic rules and suffixes
.SUFFIXES: .tex .dvi .ps .pdf

.tex.dvi:
	$(LATEX) $*
	if [ `fgrep -c $(MAY_HAVE_CHANGED) $*.log` != '' ]; then \
	    $(LATEX) $*; \
	fi
.dvi.ps:
	$(DVIPS) $* -o $*.ps
.ps.pdf:
	$(PS2PDF) $*.ps $*.pdf
# ------------------

default: $(FILE).ps

all: $(FILE).ps $(FILE).pdf

$(FILE).dvi: $(FILE).tex
	@TEXINPUTS="./texinputs:${TEXINPUTS}"; \
	export TEXINPUTS; \
	echo "TEXINPUTS=$${TEXINPUTS}"; \
	$(LATEX) $(FILE) \
	    && if [ `fgrep -c $(MAY_HAVE_CHANGED) $(FILE).log` != '' ]; then \
	           $(LATEX) $(FILE); \
	       fi \
	    && if [ `fgrep -c $(MAY_NO_BIBTEX) $(FILE).log` != '' ]; then \
	    $(BIBTEX) $(FILE); \
	    $(LATEX) $(FILE); \
	    $(LATEX) $(FILE); \
	       fi

$(FILE).pdf: $(FILE).ps
	$(PS2PDF) $(FILE).ps

$(FILE).ps: $(FILE).dvi
	$(DVIPS) $(FILE) -o $(FILE).ps

bib:
	bibtex $(FILE)

# Clean up
clean:
	rm -f $(FILE).ps* $(FILE).dvi *.aux *.toc *.log *.bbl *.blg *.nav *.snm \
	$(FILE).pdf $(FILE).out $(FILE).tex.backup $(FILE).tex~

# End of file

